Variational Inference MPC using Tsallis Divergence

In this paper, we provide a generalized framework for Variational Inference-Stochastic Optimal Control by using thenon-extensive Tsallis divergence. By incorporating the deformed exponential function into the optimality likelihood function, a novel Tsallis Variational Inference-Model Predictive Control algorithm is derived, which includes prior works such as Variational Inference-Model Predictive Control, Model Predictive PathIntegral Control, Cross Entropy Method, and Stein VariationalInference Model Predictive Control as special cases. The proposed algorithm allows for effective control of the cost/reward transform and is characterized by superior performance in terms of mean and variance reduction of the associated cost. The aforementioned features are supported by a theoretical and numerical analysis on the level of risk sensitivity of the proposed algorithm as well as simulation experiments on 5 different robotic systems with 3 different policy parameterizations.

==> RSS 2021/latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> RSS 2021/paper/algorithm.tex <==
\begin{algorithm}[t]
\caption{Tsallis Variational Inference MPC}
\begin{algorithmic}[1]
\STATE \textbf{Given:} $p(x_0)$: initial state distribution; $N$: number of policy samples; $M$: number of state  samples; $T$: MPC horizon; $T'$: number of MPC steps; $K$: optimization iterations per MPC step

\STATE Initialize $\Theta^0_0$
\STATE $\{x_0^{n,m}\}_{n,m=1}^{N,M} \sim p(x_0)$
\FOR{$t'=0$ to $T'-1$}
\FOR{$k=0$ to $K$}
\FOR{$n=1$ to $N$ \textit{in parallel}}
\FOR{$m=1$ to $M$ \textit{in parallel}}
% \FOR{$t=1$ to $T-1$}
% \STATE $u^n_t \sim \pi^k(u_t;\theta_t^k)$
% \STATE $\epsilon_t^{n,m}\sim\mathcal{N}(0, \sigma^2_\epsilon\bf{I})$
% \STATE $x^{n,m}_{t+1}=F(x_t^{n,m}, u^n_t, \epsilon_t^{n,m})$
% \ENDFOR
\STATE $X^{n,m}, U^n=f_{\text{rollout}}(x_0^{n,m}, \Theta^k_{t'})$
\STATE $J^{n,m}=f_{\text{cost}}(X^{n,m}, U^n)$
\ENDFOR
\STATE $J^n=\frac{1}{M}\sum_{m=1}^M f(\frac{J^{n,m}-\min J^{n,m}}{\max J^{n,m} - \min J^{n,m}})$
\ENDFOR
\STATE $\Theta^{k+1}_{t'}=f_{\text{update}}(\{J^n, U^n\}_{n=1}^N)$
\ENDFOR
\STATE Execute $q^K(u_{t',0})$
\STATE $\Theta^0_{t'+1}=f_{\text{recede}}(\Theta^K_{t'})$
\ENDFOR
\end{algorithmic}
\label{alg:Tsallis_VI_MPC}
\end{algorithm}

==> RSS 2021/paper/data_table.tex <==
\begin{table*}[t]
    \centering
    \caption{Comparisons of mean and standard deviation of cost against \ac{MPPI} and \ac{CEM} on different systems and policy classes. The policy classes are defined as Unimodal Gaussian (UG), Gaussian Mixture (GM), and Stein (S). Note that the negative of the reward is used for the locomotion tasks (ant and humanoid). The best mean cost and cost variance for each system-policy distribution pair is boldfaced. The mean and standard deviation reduction percentages are included to the right where positive values correspond to a reduction.}
    \begin{tabular}{
        @{}
        l
        c
        S[table-format=6.1,table-number-alignment = right,table-figures-decimal=1,table-auto-round]
        S[table-format=6.1,table-number-alignment = right,table-figures-decimal=1,table-auto-round]
        S[table-format=6.1,table-number-alignment = right,table-figures-decimal=1,table-auto-round]
        S[table-format=6.1,table-number-alignment = right,table-figures-decimal=1,table-auto-round]
        S[table-format=6.1,table-number-alignment = right,table-figures-decimal=1,table-auto-round]
        S[table-format=6.1,table-number-alignment = right,table-figures-decimal=1,table-auto-round]
        S[table-format=6.1,table-number-alignment = right,table-figures-decimal=1,table-auto-round]
        S[table-format=6.1,table-number-alignment = right,table-figures-decimal=1,table-auto-round]
        S[table-format=6.1,table-number-alignment = right,table-figures-decimal=1,table-auto-round]
        S[table-format=6.1,table-number-alignment = right,table-figures-decimal=1,table-auto-round]
        @{}
    }
    \toprule
    & & \multicolumn{2}{c}{MPPI} & \multicolumn{2}{c}{CEM}
    & \multicolumn{2}{c}{Tsallis} & \multicolumn{2}{c}{Tsallis vs MPPI} & \multicolumn{2}{c}{Tsallis vs CEM}\\
    \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12}
    {System} & {Policy} & {Mean} & {Std} & {Mean} & {Std} & {Mean} & {Std} &
    {$\Delta$Mean\%} &
    {$\Delta$Std\%} &
    {$\Delta$Mean\%} &
    {$\Delta$Std\%} \\
    % % End of header row.
    % ======== Planar Navigation ========
    \midrule
    \multirow{3.8}{*}{\begin{tabular}[c]{@{}c@{}}Planar\\Navigation\end{tabular}}
    & \begin{tabular}[c]{@{}c@{}} UG \\ \end{tabular} &
    30023.73 & 3644.07 & 34617.47 & 2523.34 & \bfseries 28714.74 & \bfseries 570.23 & 4.36 & 84.35 & 17.05 & 77.40 \\
    \cmidrule(l){2-12} 
    & \begin{tabular}[c]{@{}c@{}}GM \\ \end{tabular} &
    39313.84 & 8924.76 & 53385.30 & \bfseries 5493.97 & \bfseries 31369.22 & 5683.23 & 20.21 & 36.32 & 41.24 & -3.44 \\
    \cmidrule(l){2-12} 
    & S & 38224.95 & 5169.92 & 38847.56 & 6641.78 & \bfseries 33324.48 & \bfseries 4006.43 & 12.82 & 22.50& 14.22 & 39.68 \\
    % ======== Quadcopter ========
    \midrule
    \multirow{3.8}{*}{Quadcopter}
    & \begin{tabular}[c]{@{}c@{}}UG \\\end{tabular} &
    15266.15 & \bfseries 1374.04 & 15756.75 & 2707.08 & \bfseries 14673.40 & 1458.36 & 3.88 & -6.14 & 6.88 & 46.13 \\
    \cmidrule(l){2-12} 
    & \begin{tabular}[c]{@{}c@{}}GM \\\end{tabular} &
    22145.51 & 4007.33 & 17654.08 & 1593.86 & \bfseries 16430.56 & \bfseries 1498.24 & 25.81 & 62.61 & 6.93 & 6.0 \\
    \cmidrule(l){2-12} 
    & S &
    29238.25 & 5084.31 & 21064.73 & 2218.02 & \bfseries 15976.02 & \bfseries 1218.32 & 45.36 & 76.04 & 24.16 & 45.07 \\
    % ======== Manipulator ========
    \midrule
    \multirow{3.8}{*}{Franka}
    & \begin{tabular}[c]{@{}c@{}}UG \\\end{tabular} &
        64.17 & 8.43 & 66.37 & 18.40 & \bfseries 57.41 & \bfseries 5.53 & 10.6 & 34.5 & 13.6 & 70.1 \\
    \cmidrule(l){2-12} 
    & \begin{tabular}[c]{@{}c@{}}GM \\\end{tabular} &
        67.16 & 8.26 & 68.74 & 13.01 & \bfseries 59.15 & \bfseries 5.37 & 11.98 & 34.9 & 13.90 & 58.5 \\
    \cmidrule(l){2-12} 
    & S & 72.40 & 4.22 & 80.35 & 13.96 & \bfseries 71.77 & \bfseries 3.29 & 0.8 & 21.4 & 10.7 & 76.4 \\
    % ======== Ant ========
    \midrule
    \multirow{3.8}{*}{Ant}
    & \begin{tabular}[c]{@{}c@{}}UG\\ \end{tabular} &
        -528.7 & 54.1 & -652.6 & \bfseries 26.7 & \bfseries -692.9 & 37.2 & 31.1 & 31.3 & 6.2 & -39.0 \\
    \cmidrule(l){2-12} 
    & \begin{tabular}[c]{@{}c@{}}GM \\ \end{tabular} &
        -621.0 & 55.5 & -659.1 & 53.6 & \bfseries -663.8 & \bfseries 36.3 & 6.9 & 34.7 & 0.7 & 32.4 \\
    \cmidrule(l){2-12} 
    & S &
        -673.7 & 36.1 & -670.0 & 32.2 & \bfseries -677.4 & \bfseries 13.4 & 0.6 & 62.8 & 1.1 & 58.3 \\
    % ======== Humanoid ========
    \midrule
    \multirow{3.8}{*}{Humanoid}
    & \begin{tabular}[c]{@{}c@{}}UG\\ \end{tabular} &
        -423.79 & 233.81 & -660.80 & 208.48 & \bfseries -899.27 & \bfseries 80.09 & 112.20 & 65.74 & 36.09 & 61.58 \\
    \cmidrule(l){2-12} 
    & \begin{tabular}[c]{@{}c@{}}GM\\ \end{tabular} &
        -592.85 & 170.15 & -725.92 & 164.92 &\bfseries -738.08 & \bfseries 103.76 & 24.50 & 39.02 & 1.67 & 37.09 \\
    \cmidrule(l){2-12} 
    & S &
        -794.69 & 173.96 & -840.81 & 168.12 & \bfseries -919.67 & \bfseries 105.85 & 15.73 & 39.15 & 9.38 & 37.04 \\
    \bottomrule
    \end{tabular}
    \label{tab:data_table}
\end{table*}

==> RSS 2021/paper/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm,amsthm,mathtools}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}
\newcommand{\T}{^\mathrm{T}}
\newcommand{\tr}{\mathrm{tr}}
% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}

\newcommand{\Nb}{\mathbb{N}}
\newcommand{\Rb}{\mathbb{R}}
\newcommand{\Sb}{\mathbb{S}}
\newcommand{\Eb}{\mathbb{E}}
\newcommand{\CVaR}{\text{CVaR}}
\newcommand{\VaR}{\text{VaR}}
\newcommand{\ExP}[2]{\Eb_{{#1}}{\left[#2\right]}}

% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}
\def\calN{{\mathcal{N}}}
\def\calF{{\mathcal{F}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\logr}{\log_r}
\newcommand{\expr}{\exp_r}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}[2]{\mathcal{D}_{KL}\left({#1}\parallel {#2}\right)}
\newcommand{\TKL}[3]{\mathcal{D}_{TKL_{#1}}\left({#2}\parallel {#3}\right)}
\newcommand{\f}[2]{\mathcal{D}_f\left({#1}\parallel {#2}\right)}
\newcommand{\D}[3]{\mathcal{D}_{#1}\left({#2}\parallel {#3}\right)}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\Sr}{\mathcal{S}_r}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

% Custom command
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator\erf{erf}

\DeclarePairedDelimiter\abs{\lvert}{\rvert}
\DeclarePairedDelimiter\norm{\lVert}{\rVert}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\diag}{diag}
\let\ab\allowbreak

\newcommand{\wrapcell}[1]{\begin{tabular}[c]{@{}c@{}}#1\end{tabular}}
% Bogdan specific
\newcommand{\bogdan}[1]{\textcolor{blue}{\textbf{Bogdan:} #1}}
\newcommand{\bogdanedit}[1]{\textcolor{blue}{#1}}
\newcommand{\bogdanremove}[1]{\textcolor{blue}{\sout{#1}}}

==> RSS 2021/paper/packages.tex <==
% numbers option provides compact numerical references in the text. 
\usepackage[numbers]{natbib}
\usepackage{multicol}
\usepackage{xr-hyper}
\usepackage[bookmarks=true]{hyperref}
\usepackage{times}

\usepackage[nolist]{acronym}
\begin{acronym}
\acro{ARA}{Absolute Risk Aversion}
\acro{VI}{Variational Inference}
\acro{VI-MPC}{Variational Inference-Model Predictive Control}
\acro{SOC}{Stochastic Optimal Control}
\acro{SVGD}{Stein Variational Gradient Descent}
\acro{SS}{Stochastic Search}
\acro{MPPI}{Model Predictive Path Integral}
\acro{MPC}{Model Predictive Control}
\acro{CEM}{Cross Entropy Method}
\acro{RL}{Reinforcement Learning}
\acro{KL}{Kullback-Leibler}
\acro{EM}{Expectation Maximization}
\end{acronym}
\usepackage{hyperref}
\hypersetup{colorlinks = true,
            linkcolor = blue,
            urlcolor  = black,
            citecolor = blue,
            anchorcolor = blue}

\usepackage{url}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{algorithm}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{bm}
\usepackage{mathtools}
\usepackage{amsthm}
\usepackage{mathrsfs}
\usepackage{subcaption}
\usepackage{graphicx} % for pdf, bitmapped graphics files
\usepackage{caption}
% \usepackage{tabularx}
% \usepackage{algorithm2e}
\usepackage{algorithmic}
% \usepackage{algpseudocode}
\usepackage[nolist]{acronym}
\usepackage{bbm}
\usepackage{xcolor}
\usepackage{wrapfig}
\usepackage{siunitx}
\usepackage{multirow}
% \usepackage{todonotes}

\let\labelindent\relax
\usepackage{enumitem}

\usepackage[symbol]{footmisc}
% \usepackage{multicol}
\usepackage{float}
\usepackage[capitalise]{cleveref}
\usepackage{caption}

\usepackage{tikz}
\usepackage{etoolbox}
\usepackage{siunitx}
\usepackage{booktabs}
\usepackage{natbib}

\sisetup{detect-all}

% Robustify the bf series.
\robustify\bfseries

% Only needed for strikethrough command \sout
\usepackage{ulem}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
